Design and Characterization of 3D Printed, Open-Source Actuators for Legged Locomotion

Impressive animal locomotion capabilities are mediated by the co-evolution of the skeletal morphology and muscular properties. Legged robot performance would also likely benefit from the co-optimization of actuators and leg morphology. However, development of custom actuators for legged robots is often expensive and time consuming, which discourages roboticists from pursuing performance gains afforded by application-specific actuator optimization. This paper presents open-source designs for two quasi-direct-drive actuators with performance regimes appropriate for an 8--15 kg robot, built completely with off the shelf and 3D-printed components for less than $200 USD each. The mechanical, electrical, and thermal properties of each actuator are characterized and compared to benchmark data. Actuators subjected to 420k strides of gait data experienced only a 2% reduction in efficiency and 26 mrad in backlash growth, demonstrating viability for rigorous and sustained research applications. We present a thermal solution that nearly doubles the thermally-driven torque limits of our plastic actuator design. The performance results are comparable to traditional metallic actuators for use in high-speed legged robots of the same scale. These 3D printed designs demonstrate an approach for designing and characterizing low-cost, highly customizable, and highly reproducible actuators, democratizing the field of actuator design and enabling co-design and optimization of actuators and robot legs.

==> 3dp Actuator Arxiv/sections/1introAIM.tex <==
\section{INTRODUCTION}
\label{sec:intro}

{Bioinspired} legged robots have shown impressive agility, terrain traversal ability, and robustness \cite{minicheetah, ANYmal, SubT, azocar2020design}.
However, their performance capabilities are limited when compared to the diversity of terrestrial animals and their many forms of legged locomotion. %; current robots, while exciting, only hint at the future potential for legged platforms.
The morphological features of robots also differ greatly from their animal inspirations.
The most popular mechanical designs have maximized simplicity and generality, typically featuring identical actuators and two-link legs across the robot \cite{raw_patel2019}.

In animals, locomotor performance (\emph{i.e.}, maximum speed, acceleration, cost of transport, and maneuverability) is largely determined by the structure of the musculoskeletal system, which varies greatly across species \cite{Biewener,polly_limbs_2007}.
Analogously, morphological factors in quadrupedal robot design, such as leg shape and orientation, have been optimized to increase whole robot performance \cite{de_vincenti_control-aware_2021, raw_patel2019, ha_task-based_2016}.
Separately, actuator design has been optimized, but many still maintain generality for use in multiple leg joints \cite{Ding2017}.

In animals, selective pressures have favored the co-evolution of skeletal morphology and muscular properties to enable performance capabilities key to animal survival and success \cite{Biewener}.
Similarly, robot performance would likely benefit from coordinated optimization of leg and actuator design parameters (\textit{e.g.} motor selection, transmission ratio) \cite{chadwick2020vitruvio}.
However, traditionally-manufactured actuators for legged robots are often expensive and time-consuming to develop, usually requiring multi-axis CNC machining of custom parts. %cite something with a development budget
Despite clear performance benefits demonstrated in robots optimized for specific tasks (e.g., manufacturing, drones), upfront costs currently discourage roboticists from pursuing the performance gains afforded by co-designing application-specific robotic legs and actuators.

\begin{figure}[t]
%\vspace{-.5cm}
\begin{center}
    %\includegraphics[width=70mm]{Figures/hardware_pic.jpg}
    \includegraphics[width=1\columnwidth]{Figures/hardware.jpg}
    %\vspace{-.8cm}
    \caption{Actuator Hardware. Amber components are SLA-HT and grey components are FDM-PLA printed. A full actuator can be printed in 14 hours. A full actuator consists of one Input Assembly (primarily amber, left) and one Transmission Assembly (primarily grey, right).}
    \label{fig:photo}
\end{center}
%\vspace{-.5cm}
\end{figure}

Rapid prototyping helps reduce the cost and time for iterative and customized actuator design.
Researchers and hobbyists have leveraged 3D printing to design general-purpose actuators and transmissions \cite{novakova-marcincinova_intelligent_2011, noauthor_highgearratio_3DP_actuator,noauthor_hightorque_3DP_actuator}, including quasi-direct drive actuators \cite{noauthor_opentorque_nodate}. % actuators are mainly used in the hobbyist space with most of the actuator designs featuring high gear ratios 
To the best of our knowledge, no 3D printed actuators have been characterized to rigorously understand their performance for legged robots.
Additionally, the current designs do not quantitatively address the thermal issues or lifecycle limits that could arise from their plastic construction.
Other work has more rigorously addressed lifecycle limits for spur gears, but is limited in scope to steady-state rotation of a single gear pair \cite{zhang_physical_2020}.
%, but the plastic material likely affects durability and thermal tolerance.
% With additive manufacturing, delamination between layers may also limit the maximum shear and tension the actuator parts can experience.
% It would be useful to design an actuator specifically for legged locomotion to determine whether the 3D printing process compromises the performance of actuators for legged locomotion.

% ANOTHER POSSIBLE TAKE FOR WORKSHOPPING
% To the best of our knowledge, none of these 3D printed actuators have been characterized, so it is currently unclear the extent that the additive manufacturing process would affect the lifecycle and performance of these actuators. Additionally, the current hobbyist designs do not rigorously address the thermal issues that would arise from using plastic in these actuators and instead assume that these motors will only used in low load applications which does not hold for dynamic legged locomotion. \cite{noauthor_opentorque_nodate}  


%These designs are not ideal for legged locomotion use as the high gear ratios greatly hinder the ability to handle impacts. 
% Impact mitigation ability is a crucial consideration in the design of legged robot actuators as each step is effectively an impact \cite{impactmitigation}. 
% Though impedance control has been employed with these high gear ratio actuators to reduce impact forces, the overall performance of these systems is still inadequate for highly dynamic legged locomotion. 
% Quasi-Direct Drive actuators (cite) have been shown to effectively mitigate impacts without the need for elastic elements in the actuators. 
% Hobbyist designs for 3D printable Quasi-Direct Drive actuators are available \cite{noauthor_opentorque_nodate}, but limited in application due to lack of performance data and unsatisfactory thermal solutions for high load systems. 
\begin{figure*}[t]
%\vspace{-.5cm}
    \centering
    \includegraphics[width=\textwidth]{Figures/Design.pdf}
    %\vspace{-.8cm}
    \caption{\textbf{A} Resistive-capacitive thermal model of motor in actuator. \textbf{B} Input Assembly with airflow from fans ($F$) highlight and motor driver ($MD$) mounted; 
    motor stator ($MS$) and motor rotor ($MR$, floating) within high-temperature stereolithography printed housing (blue). 
    \textbf{C} 7.5:1 Planetary Transmission Assembly and \textbf{D} stick diagram. \textbf{E} 15:1 Bilateral Drive Transmission and \textbf{F} stick diagrams.
    Transmission symbols: Rotor-sun gear ($RSG$), planet carrier ($PC$), planet ($P$), ring gear housing ($RH$), planet level 1 \& 2 ($P12$), ring level 1 ($R1$), ring level 2 ($R2$).}
    \label{fig:mech_design}
    %\vspace{-.5cm}
\end{figure*}

To address these challenges and facilitate rapid and inexpensive actuator customization for optimized designs, we present two fully-characterized, open-source quasi-direct-drive actuators made with only off-the-shelf components and 3D printed parts.
These actuators can be made with only \$200 US in materials, commonplace 3D printers, and basic tools (Fig. \ref{fig:photo}). 
High torque output while maintaining backdrivability and low inertia potentially make these actuators well-suited for agile and robust legged robots \cite{impactmitigation, Urs2022Framework}.
The ease of reproduction and customization also make them useful for building legged robot models to study animal locomotion \cite{long2012darwin, nyakatura_reverse-engineering_2019}.
%\cite{flammang_bioinspiration_2011, gravish_robotics-inspired_2018}.
%They \talia{who? what are the useful design patterns? is this a key contribution? i'm not sure what this sentence is trying to communicate} also demonstrate a set of useful design patterns that make 3D printed 
Our characterization demonstrates that 3D printed actuators can be used directly or as fully-functioning prototypes for novel robot platforms.



We present the following key contributions:

\begin{enumerate}
%\item We establish simple application-oriented metrics for motor selection independent of transmission ratio (Section \ref{subsec:coselection}).

\item We demonstrate the viability of 3D printed actuators for legged robotics through rigorous characterization (Section \ref{sec:charmethod}).
Empirically determined mechanical, electrical, and thermal properties are presented and compared to benchmark data (Section \ref{sec:charresults});

\item We present a thermal solution for plastic actuator parts (Section \ref{subsubsec:thermaldes}) that raises thermally-driven performance limits to near-parity with metallic designs (Section \ref{subsubsec:resultthermdyn});

\item We demonstrate the durability of 3D printed actuators by measuring changes in performance over 420,000 strides of simulated gait execution (Section \ref{subsec:resultlifecycle});

\item We facilitate the rapid development of new 3D printed actuators by making the mechanical, electrical, and software designs completely free and open source. %, and 

% y describing a set of best-practices (Section \ref{subsubsec:considerations_3dp}) 

\end{enumerate}

%Harnessing 3D printing facilitates rapid development, enabling optimization of actuators on a per-joint level to expand legged robot performance regimes. 





==> 3dp Actuator Arxiv/sections/2designAIM.tex <==
%\vspace{-.2cm}
\section{Actuator Design}
\label{sec:design}



%\subsection{Design Priorities}
%\label{subsec:priorities}

Our actuators are designed for an 8--15~kg quadrupedal robot --- a useful scale for indoor testing, analogous to a small goat or dog.
At this scale, electromagnetic actuators, particularly % have proven to be the most effective style due to high availability of 
Permanent Magnet Synchronous motors (PMSMs), lend themselves to use in legged robots due to their availability in a variety of sizes, ease of control, and useful performance characteristics \cite{minitaur}. 
While Series Elastic Actuators (SEAs) have been used effectively to mitigate impact forces, improve torque fidelity, and store energy \cite{ANYmal, pratt1997stiffness, azocar2020design, ruppert2019series}, Quasi-Direct-Drive (QDD) actuators have been particularly effective at high speed, responsive locomotion \cite{minicheetah, Ding2017, pennjerboa}. 
QDD actuators can also virtually mimic the elasticity of SEAs via impedance control or other techniques \cite{Kalouche_GOAT} and achieve impact mitigation via lower output mechanical impedance (OMI) at frequencies relevant to animal locomotion \cite{impactmitigation, zhu2021design}.
% Within this category, two design patterns are prevalent: Series Elastic Actuators (SEAs) and Quasi-Direct-Drive Actuators (QDDs).

% SEAs use high-reduction transmissions to gain mechanical advantage, but include an elastic element in series to lower the back-driving mechanical impedance.
% The elastic element mitigates forces from impacts (i.e., footsteps) and allows force/torque sensing via measurement of elastic deflection, but limits responsiveness and control bandwidth \cite{pratt1997stiffness}.
% The elastic element also serves as an energy storage mechanism which helps some robots achieve low Cost of Transport (CoT) \cite{ruppert2019series}. 
% QDDs forego the elastic element and use a large motor with a low-reduction transmission to lower mechanical impedance. This pattern allows for torque estimation via motor current (which is proportional to torque) and higher responsiveness often at the cost of a lower torque ceiling \cite{impactmitigation,minitaur}.
% This torque estimation capability for actuators is referred to as proprioception (distinct from neurological proprioception), so these actuators are also sometimes referred to as proprioceptive actuators \cite{impactmitigation, seok_actuator_2012}. QDDs can also virtually mimic the elasticity of SEAs via impednace control or other techniques \cite{Kalouche_GOAT}.

%Several legged robots effectively use QDDs actuators with a breadth of control strategies and behaviors \cite{minicheetah, Ding2017, pennjerboa}. 
We seek to follow the QDD actuator design philosophy, but increase reproducibility and design flexibility by exploiting the use of 3D printing.
%This design philosophy has proven to be very effective and opens the door for a breadth of control strategies and robot behavior [cite].
Based on existing robots at the 8--15~kg scale, actuators should be capable of 5--15~Nm of torque and speeds of 15--35~rad/s with output inertia in the $10^{-4}$--$10^{-2}$~kgm$^2$ magnitude range \cite{minicheetah}.

%\vspace{-.2cm}
\subsection{Motor and Transmission Co-Selection}
\label{subsec:coselection}

For legged robots that perform highly dynamic motions, it is important that their actuators feature high torque density and power, as well as increased responsiveness and impact mitigation ability \cite{impactmitigation}. Thus motors with a high torque constant $K_T$, high motor constant $K_M$, low inertia $J_m$, and low mass $m$ are desired. To select a motor with the right balance of these properties and the appropriate transmission to complement the motor, we used the design methodology detailed in \cite{Urs2022Framework}. % High power and torque density, responsiveness, and impact mitigation capability are critical qualities for agile legged robot actuators \cite{impactmitigation}. 
% Thus, motors with a high torque constant $K_T$, high motor constant $K_M$, low inertia $J_m$, and low mass $m$ are desired.
% %Because these parameters are subject to tradeoffs, w
% We used the following selection process:
% (1) select a motor with an advantageous balance between key parameters, and 
% (2) select a transmission to make best use of the motor for the given application (\textit{i.e.}, sufficiently amplify torque while retaining speed).
% %Given the sensitivity to mass (for the sake of robot speed) and backdriving impedance (for the sake of impact force mitigation) in legged robot actuator design,
% However, the process is not purely sequential; it is important to understand which transmission styles and ratios are practical and performant while considering motors.
% To maximize accessibility, only inexpensive and readily available motors were considered. % (Table \ref{tab:motordata}). %, looking at vendors such as T-Motor, SunnySky, KDE, and iFlight. 
% %To make use of 3D printing, only d
To ensure compatibility with 3D printing manufacturing, only direct, planetary, and bilateral drive  \cite{Matsuki2019} transmissions with ratios between 1:1 and 30:1 were considered for their exclusive use of rigid elements.

\begin{table}[h]
    %\setlength\tabcolsep{3pt}
    \caption{T-Motor RI50 motor properties, summarized from \cite{Urs2022Framework}.
    %Remove U8 and 4004, move this table to results
    }
    %\vspace{-.2cm}
    \centering
    %\begin{tabular}{rcl|ccc}
    % & $  $  &  & RI50 & U8 & V4004* \\ \hline \hline
%Winding Style & $  $  &  & Wye & Delta &  \\
%Torque Constant & $ K_T $  & [Nm/A] & 0.105 & 0.14 & 0.028 \\
%Motor Constant & $ K_M $  & [Nm/W$^{\frac{1}{2}}$] & 0.12 & 0.23 & 0.041 \\
%Motor Inertia & $ J_m $  & [gm$^2$] & $9.2 \times 10^{-3}$ & 0.12 & 0.012 \\
%Mass & $ m $  & [g] & 181 & 230 & 51 \\
%Responsiveness Metric  & $ t_\omega $  & [ms] & 0.67 & 2.3 & 7.1 \\ %(\ref{eq:time_const})
%  & $ J_m / K_T^2 $  & [$\times 10^{-3}$] & 0.83 & 6.1 & 15.3 \\ \hline %(\ref{eq:scaling_J_KT})
%    \label{tab:motordata}
%    \end{tabular}
    
    \begin{tabular}{rcl|ccc}
     & $  $  &  & RI50 \\ \hline \hline
Winding Style & $  $  &  & Wye \\
Torque Constant & $ K_T $  & [Nm/A] & 0.105 \\
Motor Constant & $ K_M $  & [Nm/W$^{0.5}$] & 0.12 \\
Motor Inertia & $ J_m $  & [kgm$^2$] & $9.01 \times 10^{-6}$ \\
Mass & $ m $  & [g] & 193 \\
Responsiveness Metric  \cite{Urs2022Framework} & $ S_M $  & [ms] & 0.67 \\ %(\ref{eq:time_const})
Torque-Specific Inertia \cite{Urs2022Framework} & $ S_T $  & [g(A/N)$^2$] & 0.82 \\ \hline %(\ref{eq:scaling_J_KT})
    \label{tab:motordata}
    \end{tabular}
    
    %\vspace{-.2cm}
\end{table}


% The most popular motor for legged robots in Table \ref{tab:motordata} is the large gap-radius, exterior-rotating T-Motor U8 and ``8108'' size equivalents (iFlight EX8, SunnySky M8) \cite{minicheetah, minitaur, pennjerboa, azocar2020design}.
% The selection of this motor is motivated by physics-based dimensional scaling analysis of ideal motor models.
% This analysis suggests that, under a mass constraint, maximizing motor gap radius should be the best way to maximize $K_T$ and $K_M$ while minimizing $J_m$, which matches the best-fit trends of real motor data across a broad range of motors \cite{impactmitigation, seok_actuator_2012, Sensinger_ext_motor}.
% However, within a given performance regime (\textit{e.g.}, a particular torque and mass range), the differences between real and ideal motors can result in motor properties that deviate from the broader trend;
% we show this effect via direct evaluation of the properties of interest in the following analysis.

% % These physics-based ideal motor laws match with the best-fit trends of real motor data across a broad regime \cite{impactmitigation}.
% %However, the properties of real motors may differ slightly from those predicted by ideal motor laws.
% %in a narrow range for a given application, differences between particular motors can be more important than the trend
% % We present an analysis to identify performance gains afforded by differences between ideal and real motors.
% %While those trends hold at a broad range of motor sizes, we present an analysis to identify performance gains afforded by differences between ideal and real motors in a given range associated with an application.

% Motor properties, when combined with a transmission selection, yield effective actuator performance characteristics. The effective torque constant, $K_{Ta}$, is defined as:
% \begin{align}
%     K_{Ta} &\doteq N\times K_T
%     \label{eq:act_kt} 
% \end{align}
% in [Nm/A]; the effective motor constant, $K_{Ma}$, is defined as:
% \begin{align}
%     K_{Ma} &\doteq N\times K_M
%     \label{eq:act_km}
% \end{align}
% in [Nm/W$^{1/2}$]; and the actuator inertia, $J_a$, is defined as:
% \begin{align}
%     J_a &\doteq N^2 J_m
%     \label{eq:act_Jm}
% \end{align}
% with the transmission ratio, $N$, defined as a speed reduction.
% These equations demonstrate that there is no straightforward motor and transmission ($N$) choice that balances the tradeoff between $K_{Ta}$ and $K_{Ma}$ on one hand and $J_a$ on the other.

% However, we can arrange these quantities to simplify motor selection with metrics that conveniently do not rely on transmission selection (assuming zero transmission mass and friction):
% %To understand the relevant design trade-offs of motor selection quantitatively, we can use the following metrics, which conveniently remove the transmission selection from consideration (assuming massless transmissions with no frictional losses). 
% %These metrics are useful to understand the aforementioned intrinsic advantages of a motor:
% %\vspace{-.2cm}
% \begin{align}
%     \frac{J_a}{K_{Ma}^2} = \frac{N^2 J_m}{N^2 K_M^2} &= \frac{J_m}{K_M^2}
%     \label{eq:scaling_J_KM} \\
%     \frac{J_a}{K_{Ta}^2} = \frac{N^2 J_m}{N^2 K_T^2} &= \frac{J_m}{K_T^2}
%     \label{eq:scaling_J_KT}
% \end{align}
% Motors that minimize these ratios have an intrinsically better balance of properties for the characteristics of interest (maximizing $K_T$ and $K_M$ while minimizing $J_m$). 

% %[physical implication of these numbers is explained in eq 6-9, which translates into motor responsiveness]
% Equation (\ref{eq:scaling_J_KM}) also has a physical implication: it happens to be an approximation of a motor’s mechanical time constant of speed response to voltage change, $t_\omega$, which should be minimized to improve responsiveness:
% \begin{equation}
%     \tau_m = J_m \dot{\omega} = \frac{K_T}{R_\phi} (V_q - K_B \omega)
% \end{equation}
% %\vspace{-.2cm}
% \begin{equation}
%     J_m \Omega(s) s = \frac{K_T}{R_\phi} (V_q(s) - K_B \Omega(s))
% \end{equation}
% %\vspace{-.2cm}
% \begin{equation}
%     \Omega(s)/V_q(s) = \frac{ \frac{1}{K_B}}{\frac{R_\phi J_m}{K_T K_B} s + 1} = \frac{\frac{1}{K_B}}{ \frac{J_m}{K_M^2} s + 1}
% \end{equation}
% %\vspace{-.2cm}
% \begin{equation}
%     t_\omega = \frac{J_m}{K_M^2} \label{eq:time_const}
% \end{equation}
% where $\tau_m$ is the motor torque [Nm], $\omega$ is the motor velocity ($\Omega(s)$ in Laplace domain) [rad/s], $R_\phi$ is the motor phase resistance [$\Omega$], $V_q$ is the motor q-axis voltage ($V_q(s)$ in Laplace domain) [V], $K_B$ is the motor back-EMF constant [Vs/rad], and $s$ is the Laplace variable.

% % Consideration of the quantities in \eqref{eq:scaling_J_KM} and \eqref{eq:scaling_J_KT} is a way to understand the relative suitability of a motor for use in a QDD actuator: they encapsulate the objectives of maximizing power, torque, and responsiveness independent of transmission selection.
% This analysis does not directly consider gap radius and can be evaluated for any motor. 
The interior-rotating T-Motor RI50 is a motor that has a more useful balance between torque constant, motor constant, and inertia %(\textit{i.e.}, low ratios in (\ref{eq:scaling_J_KT}) and (\ref{eq:scaling_J_KM}), see Table \ref{tab:motordata}) 
than a dimensional scaling analysis would suggest for its small gap-radius \cite{impactmitigation, Urs2022Framework}, and is available for \$62. 
The RI50's lower $K_T$ and $K_M$ can be compensated for by a higher gear ratio%((\ref{eq:act_kt}) and (\ref{eq:act_km}))
, while still maintaining a lower reflected output inertia %(\ref{eq:act_Jm}) 
compared to an actuator with the U8 or equivalent motor \cite{Urs2022Framework}.
This advantage was clearly indicated by the $S_M$ and $S_T$ selection metrics and is likely due to a higher coil turn count and an inner-rotating geometric advantage for the stator \cite{Urs2022Framework}.
%A physics-based rationale for this advantage for the RI50 is not immediately clear and is an avenue for future work.
%Alternatively, for transmission selections that result in matching reflected inertias, the RI50 actuator will produce more torque per current input than the U8 actuator.
Leveraging this advantage, the RI50 motor was selected and paired with two different transmission styles: planetary 7.5:1, and bilateral drive 15.04:1 (abbr. 15:1), similar to the configuration in \cite{ding_design_2017}. 
These ratios yield performance regimes appropriate for an 8--15~kg quadrupedal robot based on benchmarks (Table \ref{tab:actuator_comparison}).

%\begin{table}[h]
%\setlength\tabcolsep{1pt}
%    \centering
%    \caption{Key performance metrics for our actuator and a benchmark design}
%    \begin{tabular}{r c l c c c}
% & $ $ &  & 7.5 & 15 & Mini Cheetah \\  \hline \hline
%Transmission Ratio & $ $ &  & 7.5 & 15.04 & 6 \\ 
%Transmission Style & $ $ &  & Planetary & Wolfrom & Planetary \\ 
%Eff. Torque Constant & $K_{Ta}$ & [Nm/A] & 0.79 & 1.58 & 0.84 \\ 
%Eff. Motor Constant & $K_{Ma}$ & [Nm/W$^{1/2}$] & 0.88 & 1.76 & 1.38 \\ 
%Actuator Inertia & $J_a$ & [gm$^2$] & $0.64$ & $2.2$ & $2.3$ \\ 
%Mass & $m$ & [g] &  &  & 480 \\ 
%Peak Torque (20s) & $ $ & [Nm] & 7.5 & 15 & 17 \\ 
%Peak Torque (2s) & $ $ & [Nm] & 19.1 & 38.2 &  \\ 
%Continuous Torque & $ $ & [Nm] & 4.4 & 8.8 & 6.9 \\ 
%Max Speed & $ $ & [rad/s] & 21 & 11 & 40 \\ 
%Thermal Resistance & $R_{therm}$ & [$^o$C/W] & 2.27 & 2.27 & 1.23 \\ \hline
%    \end{tabular}
%    \label{tab:actuator_proposals}
%\end{table}


%A similar actuator configuration (inrunner, 24:1) has been created by Ding et al., but with a smaller and more expensive motor.

%\subsection{Design Overview}
%\label{subsec:designover}

\subsection{Mechanical Design}
\label{subsubsec:mechdes}



All non-off-the-shelf components in the design are 3D printed. 
The majority of the parts are fused-deposition (FDM) printed with polylactic acid (PLA) plastic (Hatchbox, Pomona, CA, USA) on a Prusa MK3S+ printer (Prague, Czech Republic).
These PLA parts use approximately \$3.50 in material.
%This process and material are the most commonly available forms of 3D printing.
Though FDM-PLA parts lack mechanical strength compared to molded plastic or metals \cite{ngo2018additive}, designs that avoid stress concentrations and make best use of print orientation have proved to be sufficiently strong for the application.
Because temperatures near the motor can exceed the glass transition temperature of PLA, some parts (denoted SLA-HT below) are printed via stereolithography (SLA) in High Temp Resin with a Formlabs Form 3 printer (Formlabs, Somerville, MA). These SLA-HT parts use $\sim$\$16 in material. The actuator is split into two subassemblies (Fig. \ref{fig:mech_design}). 
The Input Assembly consists of the RI50 motor stator, cooling solution (see Sections \ref{subsubsec:thermaldes} and \ref{subsec:resultthermal}), and open-source motor driver (\$84, moteus r4.5, mjbots, Cambridge, MA, USA).  All these components are mounted to a SLA-HT motor housing.
%Three bosses key into notches on the stator, constraining its rotation.
%Three optional tabs screwed into place handle axial retention.
%The motor driver mounts directly to the back of this housing with four screws, positioning its integrated magnetic encoder directly behind the rotor.

The RI50 motor rotor is attached to the SLA-HT rotor-sun gear (RSG), which is reinforced with a steel dowel pin and carries a magnet to interact with an encoder, and also bridges the Input Assembly and Transmission Assembly.
%A steel dowel pin is pressed into the RSG to lend rigidity and strength, as several other components are supported by the RSG.
%The RSG bridges the Input Assembly and Gearbox Assembly, where it interacts with the planet gears.
All components in the Transmission Assembly apart from bearings, pins, and fasteners are FDM printed in PLA.
%The planet gears are supported by the planet carrier and rotate about dowel pins via bearings in each planet gear.
In the instance of the 7.5:1 planetary transmission, the planet carrier is itself the output.
%and is supported by one bearing in the gearbox housing and another on the RSG.
For the bilateral drive transmission, the output is the secondary ring gear.
%which is supported by one bearing in the gearbox housing and another two on the RSG.
%The planet carrier is supported by a bearing on the secondary ring gear and on the RSG.
All gears use a $30\degree$ pressure angle involute profile to increase strength \cite{rick_miller_designing_2017}.
Bearings amount to $\sim$\$15.
The two main housings register with each other on an annular boss and are axially mated together with eight screws.
%The output of both actuators is a common screw and pin interface that provides stiff coupling in all six degrees of freedom.
Fasteners and pins amount to $\sim$\$8.

The bilateral drive is a compound-planetary transmission that follows the topology commonly known as Wolfrom \cite{wolfrom_wirkungsgrad_1912}.
These transmissions can achieve very high ratios in compact packaging, but typically have low efficiency compared to multi-stage planetary transmissions of the same ratio \cite{garcia_compact_2020}. 
To overcome this challenge, we have implemented an established efficiency optimization method with some additional constraints on allowable ranges for parameters to generate gear geometry for the 15:1 transmission \cite{Matsuki2019}.

%\subsubsection{Bilateral Drive Efficiency Optimization}
%\label{subsubsec:bilateralopt}

%Certain compound planetary transmission topologies, traditionally known as Wolfrom transmissions, can achieve very high transmission ratios in compact packaging, but typically have low efficiency compared to multi-stage planetary transmissions for the same ratio \cite{Garcia et al 2020 Compact Gearboxes}.
%However, Matsuki et al. have developed a method to optimize efficiency of these transmissions (referred to as bilateral drives in their work and here) by manipulating gear geometric parameters [Matsuki et al.].
%We have implemented this method with some additional constraints on allowable ranges for parameters to generate gear geometry for the 15:1 transmission.

%The primary failure modes for FDM prints are due to shear and tension, both of which are experienced by gear boxes during use.
The design of functional and reliable 3D printed components required some special considerations. 
%Components printed with FDM are highly anisotropic, so careful consideration of print orientation was necessary to maximize strength .
FDM printed parts are strongest in the print-layer plane (\textit{i.e.}, XY plane) \cite{santana_study_2017, gorski_influence_2013}, so gears were printed with their axis parallel to the Z axis---tangential forces from torque transmission then stays in the strong plane.
Components for which not all loads can be contained in the strong plane, or where shear forces are present in the strong plane, were then reinforced by incorporating metal pins to avoid layer delamination.
Delamination due to tension was avoided by use of compression preload---this preload is generated with screws between the two halves of the planet carrier.
% When interfacing with plastic, metal screws concentrate stresses---threads tapped into plastic are especially weak.
Whenever possible, we include a pocket to embed a metallic nut with threads for bolts and screws.
Heat-set inserts are another solution for threaded holes, but they cannot be placed near the edge of parts without avoiding warping during the heat-setting process in our experience.

%Sizing for press- and slip-fit pieces with 30~{\textmu}m interference and clearance (respectively) was empirically determined by printing dedicated sample parts.
%They featured holes and pegs that spanned a range of sizes to be measured.
%Because plastic creeps, the maximum retaining force of a press fit is low -- press fits for high-stress interfaces were reinforced with glue, such as the motor rotor onto the RSG.

Geometric mating features help distribute stress and aid in assembly and disassembly.
For example, splines help prevent rotation between pieces when assembled --- the R1 element of the 15:1 transmission is torsionally retained this way (Fig. \ref{fig:mech_design}).
The two planet carrier halves have pin and socket features to ensure proper alignment (\textit{i.e}., keeping all rotational axes parallel).
% Furthermore, designing custom tooling can made it easier to grip, separate, hold in alignment, and pry apart these pieces.
Ejection ports where pins may be strategically pushed through also aided in disassembling press-fit or close-fit features.

\subsection{Thermal Design}
\label{subsubsec:thermaldes}

Quasi-direct-drive actuators require low gear-ratios and therefore low torque amplification.
Maximizing torque density then requires driving the motors with high currents, producing significant joule heating.
Thermal management is critical to allow useful continuous actuator usage and high-power peak conditions, especially with plastic components
% Plastics typically have low thermal conductivity compared to metals traditionally used in this application and can warp or weaken at high temperature
\cite{ngo2018additive, flaata2017thermal}.
Prototypes with passive cooling through plastic or adhered aluminum heatsinks proved to be insufficient to meet performance goals, so we designed an active cooling solution.

Legged robot actuators often need to exert torque without rotating (\textit{e.g.}, standing while carrying load or self-weight), so using the main actuator motor to move fans is insufficient; dedicated fans are necessary.
Two auxiliary centrifugal fans (\$5 ea, 30$\times$10mm) are mounted to the side of each actuator.
The output airflow from the fans is routed into the motor via ducting cavities in the housing (Fig. \ref{fig:mech_design}) and exhausted through ports on the other side of the motor, forcing the flow over the motor windings and rotor.
%As discussed in \ref{subsec:resultthermal} below, this solution provided the necessary thermal manage to bring actuator performance up to par with metallic designs.

% \subsection{Design Considerations for 3D Printing}
% \label{subsubsec:considerations_3dp}
% When using 3D printing, orienting the Z-plane, tramming (\textit{i.e.}, tuning the inter-axis squareness of the printer), and controlling the extrusion flow rate are standard ways to increase the precision and reliability of the parts.
% By explicitly performing these checks and calibrations, it is possible to obtain high-quality parts from cheaper FDM printer models.



% Finally, we used a thermal camera to detect areas to print in high-temperature resin.
%Additive manufacturing facilitates integral ducting for forced convection air flow to reduce thermal resistance.
%The ducting in this actuator was designed to have smooth contours, maximize cross-sectional area, and keep cross-sectional area constant throughout the ducts.
%With computational fluid dynamical modeling, the design of the ducting can likely be improved.

==> 3dp Actuator Arxiv/sections/3charmethodAIM.tex <==
\section{Characterization Methods}
\label{sec:charmethod}

%\subsection{Actuator dynamometer}
%\label{subsec:dynamometer}

To empirically determine the mechanical, electrical, and thermal properties of the actuator useful for whole-robot design and modelling, we constructed a dynamometer to conduct characterization experiments (described in \cite{Urs2022Framework}).
%The dynamometer features two actuators in opposition with outputs connected through a rotary torque sensor (TRD605-18Nm, TRS605-5Nm, Futek, Irvine, CA).
%Both actuators may act as the loading or driving actuator, and can swap roles mid-test as necessary.
%Each actuator may source from or sink power to the DC bus created by a 36~V power supply (HRP-600-36, MeanWell, New Taipei City, Taiwan) or a Zeee 30~V lithium-polymer battery (Fenggang, Dongguan, Guangdong, China).
%Power input to the dynamometer (power supply or battery) and the bidirectional power moving between the two actuators was measured with two INA260 power meters (Adafruit, New York, USA).
%The motor drivers (moteus r4.5/r4.8, mjbots, Cambridge, MA, USA) can be queried for position, velocity, q-axis current, and diagnostics over Controller Area Network-Flexible Datarate.
%A host Linux single-board computer (4B, Raspberry Pi Foundation, Cambridge, UK) commands and queries all devices and log data using custom software written in C++.
%Using CPU isolation and scheduler priority to achieve sufficient real-time performance, the program commands and queries the two drivers, samples sensors, and logs data at a maximum of 0.5-2.7~kHz, depending on which devices are in use.

%\subsection{Passive Properties}
\subsection{Motor Properties}
\label{subsec:methodpassive}
Properties of the RI50 motor were empirically determined in \cite{Urs2022Framework}. 
The methods are repeated here in brief for convenience:
\begin{itemize}
\item \textbf{Winding style:} A ``line-to-line'' current was applied through the motor to heat it while the spatial distribution was monitored with a thermal camera.
\item \textbf{Resistance ($R_\phi$):} Precision multimeter line-to-line measurement, converted to phase-frame.
\item \textbf{Inductance ($L_e$):} Precision LCR meter line-to-line measurement, converted to phase-frame.
\item \textbf{Torque Constant ($K_T$):} Various q-axis currents were commanded to the motor while it was held under stall. Actual q-axis current $i_q$ was measured by the motor driver along with torque by a transducer; a line was then fit to this data where the slope is $K_T$.
\item \textbf{Back EMF Constant ($K_B$):} The motor was back-driven by a cordless drill while the phase line-to-line voltages were measured with an oscilloscope.
\item \textbf{Motor Constant ($K_M$):} $K_M$ can then simply be calculated as $K_M= \sqrt{K_T K_B/R_{\phi}}$
\end{itemize}



% PMSM Motors typically use an iron core stator with coil windings of copper wire to generate magnetic fields.
% The windings are typically wound in one of two common styles: “Wye” and “Delta”; knowledge of the winding style is useful in motor modeling \cite{rouse motor modeling}.
% Due to the compact assembly, it is often not possible to visually observe the winding style; in this case, a thermal test is appropriate.
% While passing current between two phase terminals (``line-to-line'') to heat the windings, we observed the motor with a thermal camera (A655, Teledyne FLIR, Wilsonville, OR, USA) to visually determine the winding style, as done in \cite{lee_empirical}.%: in a Wye scheme, two windings would appear hot for every cold winding.
%Delta windings exhibit the opposite pattern.

%Line-to-line resistance was measured with a multimeter (34461A, Keysight, Santa Rosa, CA, USA), and line-to-line inductance was measured with a precision LCR meter (TMPRO 4230, Wayne Kerr, West Sussex, UK).

% For both resistance and inductance, the value between all three combinations of phase terminals (line-to-line measurements) were measured and then averaged to yield a final result, which was then converted to phase-frame (phase resistance $R_\phi$ and effective inductance $L_e$) with knowledge of the winding style, per \cite{mevey2009sensorless}.

% \subsection{Motor Coefficients}
%\label{subsec:methodconstants}

%By the Biot-Savart law, magnetic field strength, and therefore torque in a PMSM, is proportional to current.
%The torque constant, $K_T$ [Nm/A], describes the proportionality between motor torque $\tau_m$ and q-axis current $i_q$ in motors.
% To empirically determine the torque constant, $K_T$, for the RI50 motor, the motor under test was commanded with quadrature-axis current (``q-axis'', see \cite{mevey2009sensorless}) using the embedded field-oriented controller (FOC) for 5~s while mechanically stalled. 
%Torque from the transducer and measured $i_q$ data were collected.
% For each $i_q$ command 5~s test (-8 to 8~A in 1~A increments), the first and last 0.5~s of torque data were discarded to remove any transient artifacts.
%The remaining current and torque data were plotted.


%By Lenz’s Law, a back electromotive force (back EMF, or BEMF) will be generated proportional to the speed of the rotor in a PMSM.
% The back electromotive force (back EMF, or BEMF) constant, $K_B$ [Vs/rad], describes the proportionality between rotational speed and the q-axis voltage ($V_q$).
% To empirically determine $K_B$, the motor under test was back-driven by a cordless drill while the phase line-to-line voltages were measured with an oscilloscope.
%The line-to-line voltage appears as a sine wave with a frequency, $f = N_P\omega2\pi$, where $N_P$ represents the number of pole-pairs in the motors, and peak-to-peak amplitude, $V_pp = \sqrt{3} V_q$ (for a Wye winding style).

% The fundamental motor constant, $K_M$ can then simply be calculated as $K_M= \sqrt{K_T K_B/R_{\phi}}$

%\vspace{-.2cm}
\subsection{Dynamic Properties} %shorten
\label{subsec:methoddynamic}

While the motor constants describe steady-state behavior, dynamic properties must be determined to aid in system modeling and control design.
In legged robots with very light leg links, actuator dynamics may dominate leg system dynamics \cite{impactmitigation}.

% \textbf{Just cite tmech paper here.}

We determined the actuator dynamic properties via random-input testing to observe the frequency response of the system using a procedure described in detail in \cite{Urs2022Framework}.
In brief, an electrically disconnected actuator was mechanically driven with a low-pass-filtered torque signal produced by the driving actuator. 
A parametric transfer function estimate of the system was then fit to the data with a two-stage optimization procedure.
%The actuator under test was disconnected from the motor driver such that the phase leads were open circuits.
%A driving actuator was commanded with a Gaussian random process (i.e., white noise) low-pass filtered to 40~Hz input and scaled to a current command in the ranges [-0.5,0.5]/$K_{Ta}$, [-1.0,1.0]/$K_{Ta}$, and [-2.0, 2.0]/$K_{Ta}$~A.
%Torque data were collected from the torque transducer and velocity data were collected from the actuator encoder (sampled at 40kHz and filtered onboard the motor driver) together at 1100~Hz.

%These data were fit with a non-parametric model in the frequency domain via Welch’s method in the Matlab \texttt{tfestimate()} function \cite{welch_use_1967}.
%Then, a first-order parametric model was fit to the non-parametric estimate by optimizing a fit to the gain frequency response, then finally optimizing for time-domain Variance Accounted For (VAF) to obtain the final parameter estimate, both with \texttt{fmincon()}.
%We chose a time-domain analysis (VAF) for the second optimization stage as fitting in the frequency domain overemphasizes frequencies with low signal energy contribution.
The experiment was repeated without the actuator so that dynamics of the dynamometer hardware (\textit{e.g.} shaft couplers) could be subtracted away.

%\vspace{-.3cm}
\subsection{Thermal Modeling}
\label{subsec:methodthermal}
%Thermal limitations are often the driving limitations for actuators.
The temperature rise of the stator windings, which must be kept below 100 $^\circ$C to avoid premature winding thermal failure, is typically the limiting factor for actuator torque.
It is particularly critical to manage temperature rise in the primarily-plastic design, in which critical components may fail by warping due to heat.
To understand performance limitations and the benefit of the cooling solution (Section \ref{subsubsec:thermaldes}), we empirically identified a thermal model of the system.


\subsubsection{Electrical-Thermal Calibration and Measurement}
\label{subsubsec:methodthermistor}

%PMSMs use multiple windings to generate magnetic fields and torques via patterns of current flow.
%Consequently, there is a nonuniform distribution of temperatures over the motor windings.
To take temperature readings of a PMSM, thermal imaging followed by averaging over the winding visible regions is a reliable method to encapsulate spatial temperature distribution effects, unlike single-point measurements \cite{lee_empirical}.
However, the motor enclosure geometry determines air flow and blocks imaging temperature measurement.
Instead, we modeled the effect temperature has on winding electrical resistance, effectively using the motor as a thermistor.

% To calibrate the ``thermistor-effect'' behavior of the motor, we removed it from the actuator assembly to expose the windings to imaging by the thermal camera.
% While the camera collected temperature data, a voltage was applied across two of the motor phases to raise the motor temperature via Joule heating.
% An in-line power meter measured the voltage $V$ across and current $i_{bus}$ through the phases, yielding the line-to-line winding electrical resistance $R_{ll} = V/i_{bus}$.
% For each sampling instant, the motor temperature was taken to be the average temperature of all the thermal image pixels of the windings (Figure \ref{fig:thermal_bw}).
% Temperature was plotted with 50-sample averaged resistances to yield a linear fit calibration equation.
% Using this calibration, $R_{ll}$ serves as an accurate proxy measurement for true winding temperature without special consideration for the spatial temperature distribution in the motor.

To calibrate the ``thermistor-effect'' behavior of the motor, the windings were exposed to a thermal camera while a voltage was applied across two of the motor phases.
An in-line power meter measured the voltage $V$ across and current $i_{bus}$ through the phases, yielding the line-to-line winding electrical resistance $R_{ll} = V/i_{bus}$.
The average temperature of all the winding pixels (a roughly annular region in Figure \ref{fig:thermal_bw}) was plotted with 50-sample averaged resistances to yield a linear fit calibration.


\subsubsection{Thermal Dynamics}
\label{subsubsec:methodthermdyn}

%With the thermistor-effect calibration of the motor, we can take high-quality temperature measurements of the motor fully assembled in the actuator with no modifications that might influence the thermal behavior (e.g., imaging ports).
We conducted a test similar to Section \ref{subsec:methoddynamic} to identify the thermal system.
Random voltages were programmatically generated and commanded to an adjustable power supply (1687B, B\&K Precision, Yorba Linda, CA, USA), which applied the voltage across two motor phases to heat the motor.
%The same resistance measurement via Ohm's law was made, then converted to temperature via the thermistor-effect calibration described above.
The random voltages were held for 20~s before changing.
Temperature was obtained via $R_{ll}$ and the thermistor-effect calibration.
To understand the relative improvement from the fans, this experiment was conducted with and without the fans powered for one hour from a cold start.

For identification purposes, we considered the system to be the following second-order ODE corresponding to the thermal circuit in Fig. \ref{fig:mech_design} A.
The input signal was the electrical power input $P = Vi_{bus}$ (which is all translated to heat), and the output signal was the temperature rise above ambient ($T_A = 25 \degree$C) as measured via the thermistor effect:
\begin{equation} \label{eq:thermal_tf}
    \frac{T_W (s) - T_A}{P(s)}= \frac{R_{HA} + R_{WH}+ C_{HA}R_{HA}R_{WH}s}{(C_{HA}R_{HA}s + 1)(C_{WA}R_{WH}s + 1)}
\end{equation}
where the $R$ and $C$ terms are defined in Figure \ref{fig:mech_design}.

%\begin{figure}
%    \centering
%    \includegraphics[width=50mm]{Figures/thermal_circuit.pdf}
%    \caption{Thermal circuit representation of the actuator}
%    \label{fig:thermal_circuit}
%\end{figure}

\subsection{Power Efficiency}
\label{subsec:methodpower}

% Motors convert electrical power into mechanical power in positive work states (torque and velocity in the same direction), and vice versa in negative work states (torque and velocity opposed).
% Losses in power conversion happen in both the electrical (switching losses, Joule heating, etc.) and mechanical (friction) domains, and depend on velocity and torque levels.
To characterize power efficiencies for our actuators, we conducted an experiment with a loading actuator under velocity control and a driving actuator under torque control.
A set of 1838 conditions for the 7.5:1 actuator and 1568 for the 15:1 actuator across positive and negative power regimes were performed. 
Electrical power meters collected voltage and current data on the DC bus, while the torque sensor and motor driver encoders collected mechanical power data.
%Each condition resulted in a positive work efficiency for one actuator and a negative work efficiency for the other.
To manage electrical transients, the loading actuator was ramped up to speed over 0.1~s, followed by a 0.1~s delay before the driving actuator was ramped up to torque over 0.1~s. 
The condition was held for 0.8~s before ramping down in reverse order.

\subsection{Lifecycle}
\label{subsec:methodlifecycle}

Lifecycle testing of 3D-printed gears has been conducted in \cite{zhang_physical_2020}, but we employ a test that more accurately captures the transient nature of legged locomotion.
We subjected two 7.5:1 actuators to a 57 hour lifecycle test in application-like loading.
We used 106 minutes of MIT Mini-Cheetah torque and velocity data from its 12 actuators while it traversed level ground in various gaits (standing, walking, trotting).
These data were ``played back'' on the dynamometer on loop: torque data were commanded to the driving actuator (tracking through current control) while the velocity data were commanded to the loading actuator (velocity controlled).
Every 41 minutes, the playback was interrupted with interval tests to gauge wear:

\begin{enumerate}
\item Power Efficiency: The same procedure described in Section \ref{subsec:methodpower} was repeated with a total of 24 torque-velocity conditions. 
The median of the torque estimates (i.e., $i_q K_{Ta}$) from the two actuators was used in place of the torque sensor, which was uninstalled for the test.
\item Steady-State Damping: While the loading actuator was placed in an idling state (motor phases open), the driving actuator was commanded with a series of velocities. 
The ratio of motor driver torque estimate to velocity yielded an effective damping coefficient.
\end{enumerate}

%These interval tests took a total of 6 minutes and were conducted in both actuator orientations (i.e., swapping which is considered loading and driving) at each interval.
%During all of the tests, actuator torque command, velocity command, torque estimate, velocity, position, inter-actuator voltage, inter-actuator current, power supply voltage, and power supply current data were collected.


\subsection{Control Performance}
\label{subsec:methodcontrol}

PMSMs driven with FOC can use high-bandwidth current control as a proxy for torque control to enable responsive action \cite{mevey2009sensorless}.
% When current control dynamics are much faster than actuator mechanical dynamics, it is more accurate to assume instantaneous tracking of current command signals in higher-level robot control algorithms.
To characterize the current controller response, we conducted a step-response test at input magnitudes of $i_q=[1,2,3,4,5,6]$~A.
Each condition was tested for 50 trials and sampled at 2.7~kHz to generate an averaged response profile.

We also conducted a random-input command test in the same manner described for the current controller (Section \ref{subsec:methoddynamic}), but with $i_q$, commands at amplitudes of $[2.0, 4.0, 6.0]$~A (low-pass filtered to 300~Hz) with command and sampling at 2.7~kHz.
The output signal was the motor driver's current measurement.
% In the moteus driver, a position controller wraps around the current controller. 
The random-input test was repeated on the 7.5:1 actuator to characterize the position controller.
Here, actuator position commands, $\theta_a$, were the input at amplitudes of $[\pi/8, \pi/4, \pi/2, \pi]$~rad (low-pass filtered to 60~Hz) with command and sampling at 1.1~kHz.
The output signal was the motor driver angle measurement.
For both of these random-input controller tests, results were analyzed in the frequency domain via the Matlab \texttt{spa()} method in order to find the controller half-power bandwidths.

==> 3dp Actuator Arxiv/sections/4charresultsAIM.tex <==
\section{Characterization Results}
\label{sec:charresults}

Our characterization results show that the 3D printed actuators possess a favorable set of mechanical, electrical, and thermal properties despite the all-plastic, low-cost construction (Table \ref{tab:actuator_comparison}).
We present our data in comparison to a benchmark, the MIT Mini-Cheetah actuator, which is more compact, has a higher maximum speed, is deployed on a successful legged robot platform \cite{minicheetah}, and has also been adapted to other applications \cite{zhu2021design}. 
%The Mini-Cheetah actuator is more compact, higher speed, and has proven to be a highly successful design, but our designs perform well despite the all-plastic, low-cost construction. 
Although 2\% of the Mini-Cheetah velocity data used for lifecycle testing (Section \ref{subsec:methodlifecycle}, \ref{subsec:resultlifecycle}) exceeded the top speed of our actuator, other legged robots perform well in this lower speed regime \cite{ANYmal}.

Lifecycle testing on the 7.5:1 actuator revealed a key finding: the actuators are capable of demanding usage for a sustained period of time; the tested actuators did not experience any failures over the course of the 57 hour test. 
All intervals are reported to 95\% confidence ($2\sigma$) unless otherwise noted.

%\captionsetup[table]{skip=5pt plus 0.01pt}
\begin{table}[]
%\begin{minipage}[t][7cm]{\columnwidth}
    %\setlength\belowcaptionskip{0pt}
    \setlength\tabcolsep{1.4pt}
    %%\vspace{-.2cm}
    %\setlength{\skip\footins}{0.1cm}
    %\setlength{\footnotesep}{0.1cm}
    %\centering
    \begin{center}
        \caption{Key actuator performance metrics. Peak torques are thermally driven; maximum tested torques are lower. Note: Mini Cheetah (``MC'') peak torque duration was not provided}
        %%\vspace{-.2cm}
        \begin{tabular}{r c l | c c c}
 & $ $ &  & 7.5 & 15 & MC \cite{minicheetah} \\  \hline \hline
Transmission Ratio & $ $ &  & 7.5:1 & 15.04:1 & 6:1 \\ 
Transmission Style & $ $ &  & Planetary & Wolfrom & Planetary \\ 
Eff. Torque Const. & $K_{Ta}$ & [Nm/A] & 0.79 & 1.58 & 0.84 \\ 
Eff. Motor Const. & $K_{Ma}$ & [Nm/W$^{\frac{1}{2}}$] & 0.88 & 1.76 & 1.38 \\ 
Actuator Inertia & $J_a$ & [gm$^2$] & $0.64$ & $2.2$ & $2.3$ \\ 
Mass & $m$ & [g] & 482 & 536 & 480 \\ 
Diameter $\times$ Length & & [mm] & $90\times70$ & $90\times90$ & $96\times40$ \\ 
Peak Torque (20s) & $ $ & [Nm] & 7.5 & 15 & \multirow{2}{*}{17} \\ 
Peak Torque (2s) & $ $ & [Nm] & 19.1 & 38.2 &  \\ 
Continuous Torque & $ $ & [Nm] & 4.4 & 8.8 & 6.9 \\ 
Max Speed & $ $ & [rad/s] & 21 & 11 & 40 \\ 
Thermal Resistance & $R_{th}$ & [$^\circ$C/W] & \multicolumn{2}{c}{2.27} & 1.23 \\ \hline
        \label{tab:actuator_comparison}
        \end{tabular}
    \end{center}
    
%\end{minipage}
%%\vspace{-.2cm}
\end{table}


	


%\subsection{Passive Properties}
\subsection{Motor Properties}
\label{subsec:resultpassive}
The results from \cite{Urs2022Framework} are summarized here for convenience:

\begin{itemize}
\item \textbf{Winding style:} Wye.
\item \textbf{Resistance ($R_\phi$):} $R_\phi = 705\pm 3$ m$\Omega$
\item \textbf{Inductance ($L_e$):} $L_e = 2559\pm 2$ {$\mu$}H
\item \textbf{Torque Constant ($K_T$):} $K_T = 0.105\pm 0.002$ Nm/A
\item \textbf{Back EMF Constant ($K_B$):} $K_B = 0.094\pm 0.002$ Vs/rad
\item \textbf{Motor Constant ($K_M$):} $K_M = 0.118 \pm 0.003$ Nm/W$^{1/2}$
\end{itemize}

% Thermal tests revealed that the winding style for the RI50 motor is the Wye winding style by the pattern of eight hot windings to four cold (Fig. \ref{fig:thermal_bw}A).
% Electrical measurements yielded a phase resistance of $R_\phi = 705\pm 3$ m$\Omega$ and an effective inductance of $L_e = 2559\pm 2$ {$\mu$}H.

%\subsection{Motor Coefficients}
%\label{subsec:resultconstants}
% The gradient of a line fit to the torque-current data yielded a torque constant of $K_T = 0.105\pm 0.002$ Nm/A.
% The gradient of a line fit to the voltage-speed data yielded a BEMF constant of $K_B = 0.094\pm 0.002$ Vs/rad. % via an average over several speeds.
For ideal PMSMs, $K_T = K_B$ on the q-axis; our slight deviations likely resulted from imperfectly sinusoidal back-EMF profiles.
% With these values for $K_T$ and $K_B$, we can then obtain the value of the fundamental motor constant ($K_M$) as 0.118$\pm 0.003$ Nm/W$^{1/2}$.
%\\
%test\\
%test\\
%test\\
%test\\
%test

\subsection{Dynamic Properties}
\label{subsec:resultdynamic}

The frequency domain non-parametric estimate and high coherence of $>0.9$ up to 40~Hz (Fig. \ref{fig:mech_sysid}) suggested that the torque and velocity data could be explained by a first-order linear model:
\begin{equation}
    \frac{\Omega (s)}{ T_b (s)} = \frac{1}{J_a s + B_a}
    \label{eq:mech_dyn_model}
\end{equation}
where $\Omega(s)$ is actuator angular velocity, $T_b (s)$ is backdriving torque, $J_a$ is actuator output inertia [kgm$^2$], $B_a$ is actuator viscous damping [Nms/rad], and $s$ is the Laplace variable.
The following parameters resulted from fitting the model: the actuator inertia $J_a$ was estimated as $(6.37 \pm 0.92) \times 10^{-4}$ kgm$^{2}$ for the 7.5:1 transmission and $(2.22 \pm 0.10) \times 10^{-3} $ kgm$^2$ for the 15:1 transmission.
The goodness of fit is evaluated with the Variance Account For (VAF) metric.
The parametric fit showed $92\%-98\%$ VAF, indicating a high-quality parameter estimation, and the estimates lined up very closely to the predictions from the equation for actuator inertia, $J_a$:
\begin{equation}
    J_a \doteq N^2 J_m
    \label{eq:act_Jm}
\end{equation}
where the transmission ratio, $N$, represents a speed reduction and $J_m$ represents motor inertia (found in \cite{Urs2022Framework}).

\begin{figure}
%%\vspace{-.2cm}
\begin{center}
    \includegraphics[width=.95\columnwidth]{Figures/mech_sysid.pdf}
    %%\vspace{-.2cm}
    \caption{Mechanical System ID Frequency Response and Coherence. Legend indicated input amplitude and Variance Account For goodness of fit. The confidence intervals for the $J$ and $B$ are 2 standard deviations of identified $J$ and $B$ across input magnitudes}
    \label{fig:mech_sysid}
\end{center}
%%\vspace{-.5cm}
\end{figure}


The drop in the model fit quality above 40Hz (Fig. \ref{fig:mech_sysid}) coincides with the cutoff frequency of the low-pass filter applied to the system input (\ref{subsec:methoddynamic}).
The model overall sufficiently explains the actuator mechanical dynamics, especially for application in legged robots, in which leg and torso dynamics are typically slower than 40Hz.
%The VAF values indicate the identified models sufficiently explain the data.

%Inertia can also be directly estimated via empirical measurements.
%Since the RI50 motor is frameless, the rotor can be independently massed.
%Approximating it as a thin ring, the inertia of just the rotor is $5.4\times10^{-4}$ kgm$^2$. This figure matches well with the frequency domain analysis, considering that the analysis includes inertial contributions from bearing races and the RSG structure and is therefore slightly higher.
%%\vspace{-.2cm}
\subsection{Thermal Modeling}
\label{subsec:resultthermal}

\subsubsection{Electrical-Thermal Calibration and Measurement}
\label{subsubsec:resultthermistor}
Winding temperature $\overline{T_w}$ [$\degree$C] and resistance $R_{ll}$ varied linearly: 
\begin{equation}
    \overline{T_w} = 139.564R_{ll} - 177.826
\end{equation}
with $R^2 = 0.99$.

This relationship can also be stated as a 0.51\% increase in resistance per \degree C, which is similar to common values for pure copper (the winding material) of 0.43\%/\degree C \cite{noauthor_resistivity_nodate}. 
Discrepancies are due to incorporating the non-heated winding temperature into the temperature average, and potentially the enamel coating on the windings and non-copper elements in the composition. 


\begin{figure}
%%%\vspace{-.2cm}
\begin{center}
\includegraphics[width=.9\columnwidth]{Figures/actuator_heat1.pdf}
%%\vspace{-.2cm}
    \caption{\textbf{(A)} Averaged thermal image over 50 frames of motor during electrical-thermal calibration. Eight of the twelve windings appear hotter than the rest, indicating a Wye winding style. \textbf{(B)} A plot showing the peak duration any current can be sustained predicted using the thermal model. A 9.2 A peak may be sustained for 20s or a 22 A peak may be sustained for 2s without exceeding temperature limits.}
    \label{fig:thermal_bw}
\end{center}
\end{figure}

\subsubsection{Thermal Dynamics}
\label{subsubsec:resultthermdyn}

Random-input thermal testing revealed that the cooling fans provide an approximately 3.5$\times$ cooling advantage, bringing performance limits to near parity with metallic actuators \cite{minicheetah, lee_empirical}.
A transfer function model (\ref{eq:thermal_tf}) fit to the thermal data yielded the system parameters in Table \ref{tab:therm_terms}; the total thermal resistance $R_{th}$ was 2.27 $^\circ$C/W.

\begin{table}
%%\vspace{-.2cm}
\begin{center}
\caption{Thermal Model Parameters}
%%\vspace{-.2cm}
    \begin{tabular}{ c c | c c } 
        & & Fan & No Fan  \\
        \hline \hline
        $R_{WH}$ & [\degree C/W]  & 0.828 & 1.09  \\
        $R_{HA}$ & [\degree C/W]  & {1.44} & {6.68}  \\
        $C_{WH}$ & [J/\degree C]  & 15.9 & 18.4 \\
        $C_{WA}$ & [J/\degree C]  & 146 & 138 \\
        \label{tab:therm_terms}
    \end{tabular}
    
\end{center}

%%%\vspace{-.8cm}
\end{table}

The 3.5$\times$  reduction in $R_{th}$ with the fans nearly doubles the amount of continuous current that can be safely dissipated, corresponding to a similar near doubling in actuator torque capabilities.
%Peak current capabilities are illustrated in Fig. ; the model predicts a sustained 20s peak of $i_q = 9.2$~A (about 1 Nm at the motor before transmission) will not bring the winding temperature above 100 \degree C.
The identification allows us to establish limits (Fig. \ref{fig:thermal_bw}B) and shows that the thermal capacitances with the fans on or off are very similar, as expected.

% \begin{figure}
%     \centering
%     \includegraphics[width=60mm]{Figures/thermal_limits_grid_notitle.eps}
%     \caption{The thermal model predicts the peak duration any current can be sustained. 
%     A 9.2 A peak may be sustained for 20s or a 22 A peak may be sustained for 2s without exceeding temperature limits.}
%     \label{fig:thermal_limits}
% \end{figure}

%With the fans blowing cool ambient air directly over the windings, a resistive path between the windings and the ambient air may have been an appropriate addition to the model.
%However, the simpler model very well explains the data, and the total resistance would be approximately the same regardless.

\subsection{Power Efficiency}
\label{subsec:resultpower}

Power efficiency testing yielded trends that match up well with the literature for other actuators \cite{lee_empirical}: efficiency is high at high speeds and low torques, but efficiency is reduced at low speed and high torque regimes by joule heating losses, which scale with $i_q^2$ and therefore $\tau_m^2$ (Fig. \ref{fig:power}).

\begin{figure}
%%\vspace{-.2cm}
\begin{center}
    \includegraphics[trim=0.2cm 0.0cm 0.1cm 0.0cm, clip,width=.95\columnwidth]{Figures/efficiency_dual_final_notitle_fat15_titleinset_tall.eps}
    %%\vspace{-.2cm}
    \caption{Efficiency map of the two actuator designs. 
    In slower and higher-torque regimes, the 15:1 transmission is more efficient. 
    In the positive work quadrant ($\tau_a>0$), efficiency is the mechanical output divided by the electric input power.
    In the negative work quadrant, the definition is inverted.
    Negative efficiencies imply actuator sinks power from both the electrical and mechanical sides. 
    Efficiencies $<-1$ are black. }
    \label{fig:power}
\end{center}
\end{figure}

\subsection{Lifecycle}
\label{subsec:resultlifecycle}

Lifecycle testing yielded highly positive results: in total, two 7.5:1 actuators were tested with gait-like test conditions for 57 hours with no failures and only limited performance degradation.
This length of time corresponds to $\sim$420,000 strides of Mini-Cheetah in the source data. 

The power efficiency interval tests (see Section \ref{subsec:methodpower}) revealed a clear trend: positive work efficiency steadily dropped for the first 8--10 hours of testing before leveling-off at a 3.5\% lower value (Fig. \ref{fig:lifecycle_eff}).
As testing went on, fine plastic dust built up in the transmission, potentially increasing friction up to a saturation point, causing a drop-then-level trend.
The efficiency then rebounded to near-original values, suggesting the presence of a slower process, such as breaking-in of parts or bearings.


\begin{figure}
%%\vspace{-.2cm}
\begin{center}
\includegraphics[trim=0.2cm 0.0cm 0.2cm 0.0cm, clip, width=.9\columnwidth]{Figures/lifecycle_efficiency_a1_a2_notitle_grey_nobox_pc.pdf}
%%\vspace{-.2cm}
    \caption{Average positive work efficiencies during the 57 hour lifecycle test of two 7.5:1 actuators. 
    An initial drop in efficiency of both actuators occurs over 8-10 hours before a leveling off, followed by a rebound to near original levels.}
    \label{fig:lifecycle_eff}
\end{center}
%%\vspace{-.5cm}
\end{figure}

The damping interval tests showed approximately constant damping coefficients: for a control input of 2.5~rad/s, the damping coefficient was $76\pm 12$~mNms/rad and for 5.0 rad/s, it was $41\pm 8$~mNms/rad without a clear trend.
%The standard deviation in the damping coefficient over the 7 second condition duration also remained approximately constant (XX$\pm$XX Nms/rad) over the XX hours of the test, indicating negligible change in the consistency of actuator rotation.

For the gait data playback and the interval tests, encoder data from both sides of the dynamometer were collected.
Assuming no encoders drift or errors, differences between the encoder readings must be due to torsional flexion and backlash.
We observed a maximum of 56~mrad difference in the first hour, which grew to 82~mrad in the last hour.
Assuming that the Young’s modulus of the components did not change during the test, this 26~mrad growth in discrepancy must be entirely due to an increase in backlash (average of 13~mrad per actuator).
The rate of backlash growth was approximately linear at a rate of $250\pm 30$~{$\mu$}rad/hr per actuator.


\subsection{Control Performance}
\label{subsec:resultcontrol}

Step-response tests of the motor driver's built-in manually-tuned current controller yielded a rise time of $2.65\pm 1.88$~ms (Fig. \ref{fig:step_response}A)
The random-input frequency response indicated a half-power bandwidth of $102\pm1$~Hz for the current controller (Fig. \ref{fig:step_response}B) and $11-30$ Hz for the position controller (plot omitted).
The current controller bandwidth is lower than comparable actuators, likely due to the high motor inductance $L_e$. 
%For both controllers, it is likely that faster responses could be achieved with more aggressive tuning. 

\begin{figure}
\begin{center}
\includegraphics[width=.9\columnwidth]{Figures/step_response.pdf}
%%\vspace{-.2cm}
    \caption{(A) Step response of q-axis current controller with an average rise time of 2.65ms (B) Frequency domain current control response at 3 input amplitudes, with with a half-power bandwidth $f_c$ of 102~Hz.}
    \label{fig:step_response}
\end{center}
%%\vspace{-.5cm}
\end{figure}

==> 3dp Actuator Arxiv/sections/6discussionAIM.tex <==
\section{Discussion}
\label{sec:discussion}

We present a full characterization of the mechanical, thermal and electrical properties of two open-source, fully 3D printed, quasi-direct drive actuators. 
With our thermal solution, actuator mechanical torque capabilities were comparable to metallic actuators currently used for small quadrupedal robots% like the Mini-Cheetah
, but with a significantly lower inertia \cite{minicheetah, lee_empirical}.
%Maximum actuator speeds are lower than the benchmark, but only 2\% of Mini-Cheetah velocity data used for lifecycle testing exceeded the top speed.
Life-cycle testing of the 7.5:1 planetary transmission prototype for 420,000 strides (57~hrs) revealed little increase in wear and backlash---after a minor drop in the first 10~hrs, efficiency rebounded to original levels.
This pattern suggests a relatively quick rise in friction until saturation, until a slower break-in process became apparent; nylon gears exhibit a similar process \cite{zhang_physical_2020}. 

Our 3D printed actuator designs reduce time and cost barriers, thereby contributing to the growing field of open-source robot development \cite{azocar2020design, grimminger_open_2020}. 
These two designs exemplify the reliability, high performance, and durability of 3D printed actuators at multiple scales.
Bio-inspired designers can extend this work to create actuators and robots that mimic a broad range of animal capabilities \cite{Urs2022SICB} ,  %applications and configurations
while being confident that they can withstand rigorous and sustained use in research settings.
We plan to develop future versions with transmission ratios optimized for particular legged robot tasks and 3D printed series-elastic actuators. 
% We also hope to make a series-elastic version of this actuator and characterize its performance relative to literature benchmarks.

% Traditionally, plastic actuators often experience thermal issues which limit their overall performance. We present a thermal solution presented gives peak actuator thermal performance on par with metallic counterparts and circumvents these issues. pen source design and low cost democratizes actuator design and eliminates the high costs associated with co-designing actuators with robot leg morphology. Makes a strong case for the rapid and iterative design process.
% \begin{enumerate}
% \item High performance coupled with enhanced durability shows real promise for 3D printed actuators for rigorous and sustained use in research settings
% \item The thermal solution presented gives peak actuator thermal performance on par with metallic counterparts and circumvents previous issues with plastic actuators
% \item Open source design and low cost democratizes actuator design and eliminates the high costs associated with co-designing actuators with robot leg morphology. Makes a strong case for the rapid and iterative design process.

% \end{enumerate}

% Further pursuits (Next steps)


% We maximized the forward- and backward-driving efficiencies of a type-3K compound planetary gearbox and tested the
% performances of a prototype gearbox.
% The prototype gearbox achieved 89.0% forward-driving efficiency, 85.3% backward-driving efficiency, and a 0.020-N·m
% reverse-drive starting torque. We also developed prototype gearboxes with gear ratios between 1/48.7 and 1/378.5. All of these
% prototypes were manually backdrivable. Our bilateral drive gears
% are expected to be employed in cooperative robots. However,
% increasing gear ratio increases the apparent inertia [22]. As the
% future work, we will investigate the effects of this apparent
% inertia. In future, we plan to develop the actuator with this
% bilateral drive gear for cooperative robots.

% \begin{enumerate}
% \item Make a series elastic version of this actuator
% \item Make a smaller version of this actuator optimized for drones 

% \end{enumerate}



% rehash the 4 contributions

% rapid/iterative design process

% use for legged robots

% \subsection{Conclusion and Next Steps}
% %repeating lifecycle test for 15:1 design
% %frequency domain representation of controller performance

% series-elastic variant
% smaller version? for drones?

% \label{subsec:conclusion}
